GWTC-3: Compact Binary Coalescences Observed by LIGO and Virgo During the Second Part of the Third Observing Run

The third Gravitational-Wave Transient Catalog (GWTC-3) describes signals detected with Advanced LIGO and Advanced Virgo up to the end of their third observing run. Updating the previous GWTC-2.1, we present candidate gravitational waves from compact binary coalescences during the second half of the third observing run (O3b) between 1 November 2019, 15:00 UTC and 27 March 2020, 17:00 UTC. There are 35 compact binary coalescence candidates identified by at least one of our search algorithms with a probability of astrophysical origin $p_\mathrm{astro} > 0.5$. Of these, 18 were previously reported as low-latency public alerts, and 17 are reported here for the first time. Based upon estimates for the component masses, our O3b candidates with $p_\mathrm{astro} > 0.5$ are consistent with gravitational-wave signals from binary black holes or neutron star-black hole binaries, and we identify none from binary neutron stars. However, from the gravitational-wave data alone, we are not able to measure matter effects that distinguish whether the binary components are neutron stars or black holes. The range of inferred component masses is similar to that found with previous catalogs, but the O3b candidates include the first confident observations of neutron star-black hole binaries. Including the 35 candidates from O3b in addition to those from GWTC-2.1, GWTC-3 contains 90 candidates found by our analysis with $p_\mathrm{astro} > 0.5$ across the first three observing runs. These observations of compact binary coalescences present an unprecedented view of the properties of black holes and neutron stars.

==> PE_table_with_cuts.tex <==
\begin{ruledtabular}\begin{tabular}{l c c c c c c c c c c c}
Event & $\underset{\displaystyle (M_\odot)}{M}$ & $\underset{\displaystyle (M_\odot)}{\mathcal{M}}$ & $\underset{\displaystyle (M_\odot)}{m_1}$ & $\underset{\displaystyle (M_\odot)}{m_2}$ & $\chi_\mathrm{{eff}}$ & $\underset{\displaystyle ({\rm Gpc})}{D_\mathrm{L}}$ & $z$ & $\underset{\displaystyle (M_\odot)}{M_\mathrm{f}}$ & $\chi_\mathrm{f}$ & $\underset{\displaystyle (\mathrm{deg}^2)}{\Delta\Omega}$ & $\mathrm{SNR}$\\ \hline
\FULLNAME{GW191103A} & $\totalmasssourceuncert{GW191103A}$ & $\chirpmasssourceuncert{GW191103A}$ & $\massonesourceuncert{GW191103A}$ & $\masstwosourceuncert{GW191103A}$ & $\chieffinfinityonlyprecavguncert{GW191103A}$ & $\luminositydistanceuncert{GW191103A}$ & $\redshiftuncert{GW191103A}$ & $\finalmasssourceuncert{GW191103A}$ & $\finalspinuncert{GW191103A}$ & $\skyarea{GW191103A}$ & $\networkmatchedfiltersnrIMRPuncert{GW191103A}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW191105C} & $\totalmasssourceuncert{GW191105C}$ & $\chirpmasssourceuncert{GW191105C}$ & $\massonesourceuncert{GW191105C}$ & $\masstwosourceuncert{GW191105C}$ & $\chieffinfinityonlyprecavguncert{GW191105C}$ & $\luminositydistanceuncert{GW191105C}$ & $\redshiftuncert{GW191105C}$ & $\finalmasssourceuncert{GW191105C}$ & $\finalspinuncert{GW191105C}$ & $\skyarea{GW191105C}$ & $\networkmatchedfiltersnrIMRPuncert{GW191105C}$\\
\FULLNAME{GW191109A} & $\totalmasssourceuncert{GW191109A}$ & $\chirpmasssourceuncert{GW191109A}$ & $\massonesourceuncert{GW191109A}$ & $\masstwosourceuncert{GW191109A}$ & $\chieffinfinityonlyprecavguncert{GW191109A}$ & $\luminositydistanceuncert{GW191109A}$ & $\redshiftuncert{GW191109A}$ & $\finalmasssourceuncert{GW191109A}$ & $\finalspinuncert{GW191109A}$ & $\skyarea{GW191109A}$ & $\networkmatchedfiltersnrIMRPuncert{GW191109A}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW191113B} & $\totalmasssourceuncert{GW191113B}$ & $\chirpmasssourceuncert{GW191113B}$ & $\massonesourceuncert{GW191113B}$ & $\masstwosourceuncert{GW191113B}$ & $\chieffinfinityonlyprecavguncert{GW191113B}$ & $\luminositydistanceuncert{GW191113B}$ & $\redshiftuncert{GW191113B}$ & $\finalmasssourceuncert{GW191113B}$ & $\finalspinuncert{GW191113B}$ & $\skyarea{GW191113B}$ & $\networkmatchedfiltersnrIMRPuncert{GW191113B}$\\
\FULLNAME{GW191126C} & $\totalmasssourceuncert{GW191126C}$ & $\chirpmasssourceuncert{GW191126C}$ & $\massonesourceuncert{GW191126C}$ & $\masstwosourceuncert{GW191126C}$ & $\chieffinfinityonlyprecavguncert{GW191126C}$ & $\luminositydistanceuncert{GW191126C}$ & $\redshiftuncert{GW191126C}$ & $\finalmasssourceuncert{GW191126C}$ & $\finalspinuncert{GW191126C}$ & $\skyarea{GW191126C}$ & $\networkmatchedfiltersnrIMRPuncert{GW191126C}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW191127B} & $\totalmasssourceuncert{GW191127B}$ & $\chirpmasssourceuncert{GW191127B}$ & $\massonesourceuncert{GW191127B}$ & $\masstwosourceuncert{GW191127B}$ & $\chieffinfinityonlyprecavguncert{GW191127B}$ & $\luminositydistanceuncert{GW191127B}$ & $\redshiftuncert{GW191127B}$ & $\finalmasssourceuncert{GW191127B}$ & $\finalspinuncert{GW191127B}$ & $\skyarea{GW191127B}$ & $\networkmatchedfiltersnrIMRPuncert{GW191127B}$\\
\FULLNAME{GW191129G} & $\totalmasssourceuncert{GW191129G}$ & $\chirpmasssourceuncert{GW191129G}$ & $\massonesourceuncert{GW191129G}$ & $\masstwosourceuncert{GW191129G}$ & $\chieffinfinityonlyprecavguncert{GW191129G}$ & $\luminositydistanceuncert{GW191129G}$ & $\redshiftuncert{GW191129G}$ & $\finalmasssourceuncert{GW191129G}$ & $\finalspinuncert{GW191129G}$ & $\skyarea{GW191129G}$ & $\networkmatchedfiltersnrIMRPuncert{GW191129G}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW191204A} & $\totalmasssourceuncert{GW191204A}$ & $\chirpmasssourceuncert{GW191204A}$ & $\massonesourceuncert{GW191204A}$ & $\masstwosourceuncert{GW191204A}$ & $\chieffinfinityonlyprecavguncert{GW191204A}$ & $\luminositydistanceuncert{GW191204A}$ & $\redshiftuncert{GW191204A}$ & $\finalmasssourceuncert{GW191204A}$ & $\finalspinuncert{GW191204A}$ & $\skyarea{GW191204A}$ & $\networkmatchedfiltersnrIMRPuncert{GW191204A}$\\
\FULLNAME{GW191204G} & $\totalmasssourceuncert{GW191204G}$ & $\chirpmasssourceuncert{GW191204G}$ & $\massonesourceuncert{GW191204G}$ & $\masstwosourceuncert{GW191204G}$ & $\chieffinfinityonlyprecavguncert{GW191204G}$ & $\luminositydistanceuncert{GW191204G}$ & $\redshiftuncert{GW191204G}$ & $\finalmasssourceuncert{GW191204G}$ & $\finalspinuncert{GW191204G}$ & $\skyarea{GW191204G}$ & $\networkmatchedfiltersnrIMRPuncert{GW191204G}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW191215G} & $\totalmasssourceuncert{GW191215G}$ & $\chirpmasssourceuncert{GW191215G}$ & $\massonesourceuncert{GW191215G}$ & $\masstwosourceuncert{GW191215G}$ & $\chieffinfinityonlyprecavguncert{GW191215G}$ & $\luminositydistanceuncert{GW191215G}$ & $\redshiftuncert{GW191215G}$ & $\finalmasssourceuncert{GW191215G}$ & $\finalspinuncert{GW191215G}$ & $\skyarea{GW191215G}$ & $\networkmatchedfiltersnrIMRPuncert{GW191215G}$\\
\FULLNAME{GW191216G} & $\totalmasssourceuncert{GW191216G}$ & $\chirpmasssourceuncert{GW191216G}$ & $\massonesourceuncert{GW191216G}$ & $\masstwosourceuncert{GW191216G}$ & $\chieffinfinityonlyprecavguncert{GW191216G}$ & $\luminositydistanceuncert{GW191216G}$ & $\redshiftuncert{GW191216G}$ & $\finalmasssourceuncert{GW191216G}$ & $\finalspinuncert{GW191216G}$ & $\skyarea{GW191216G}$ & $\networkmatchedfiltersnrIMRPuncert{GW191216G}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\textit{\FULLNAME{GW191219E}} & $\totalmasssourceuncert{GW191219E}$ & $\chirpmasssourceuncert{GW191219E}$ & $\massonesourceuncert{GW191219E}$ & $\masstwosourceuncert{GW191219E}$ & $\chieffinfinityonlyprecavguncert{GW191219E}$ & $\luminositydistanceuncert{GW191219E}$ & $\redshiftuncert{GW191219E}$ & $\finalmasssourceuncert{GW191219E}$ & $\finalspinuncert{GW191219E}$ & $\skyarea{GW191219E}$ & $\networkmatchedfiltersnrIMRPuncert{GW191219E}$\\
\FULLNAME{GW191222A} & $\totalmasssourceuncert{GW191222A}$ & $\chirpmasssourceuncert{GW191222A}$ & $\massonesourceuncert{GW191222A}$ & $\masstwosourceuncert{GW191222A}$ & $\chieffinfinityonlyprecavguncert{GW191222A}$ & $\luminositydistanceuncert{GW191222A}$ & $\redshiftuncert{GW191222A}$ & $\finalmasssourceuncert{GW191222A}$ & $\finalspinuncert{GW191222A}$ & $\skyarea{GW191222A}$ & $\networkmatchedfiltersnrIMRPuncert{GW191222A}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW191230H} & $\totalmasssourceuncert{GW191230H}$ & $\chirpmasssourceuncert{GW191230H}$ & $\massonesourceuncert{GW191230H}$ & $\masstwosourceuncert{GW191230H}$ & $\chieffinfinityonlyprecavguncert{GW191230H}$ & $\luminositydistanceuncert{GW191230H}$ & $\redshiftuncert{GW191230H}$ & $\finalmasssourceuncert{GW191230H}$ & $\finalspinuncert{GW191230H}$ & $\skyarea{GW191230H}$ & $\networkmatchedfiltersnrIMRPuncert{GW191230H}$\\
\textit{\FULLNAME{200105F}} & $\totalmasssourceuncert{200105F}$ & $\chirpmasssourceuncert{200105F}$ & $\massonesourceuncert{200105F}$ & $\masstwosourceuncert{200105F}$ & $\chieffinfinityonlyprecavguncert{200105F}$ & $\luminositydistanceuncert{200105F}$ & $\redshiftuncert{200105F}$ & $\finalmasssourceuncert{200105F}$ & $\finalspinuncert{200105F}$ & $\skyarea{200105F}$ & $\networkmatchedfiltersnrIMRPuncert{200105F}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW200112H} & $\totalmasssourceuncert{GW200112H}$ & $\chirpmasssourceuncert{GW200112H}$ & $\massonesourceuncert{GW200112H}$ & $\masstwosourceuncert{GW200112H}$ & $\chieffinfinityonlyprecavguncert{GW200112H}$ & $\luminositydistanceuncert{GW200112H}$ & $\redshiftuncert{GW200112H}$ & $\finalmasssourceuncert{GW200112H}$ & $\finalspinuncert{GW200112H}$ & $\skyarea{GW200112H}$ & $\networkmatchedfiltersnrIMRPuncert{GW200112H}$\\
\FULLNAME{GW200115A} & $\totalmasssourceuncert{GW200115A}$ & $\chirpmasssourceuncert{GW200115A}$ & $\massonesourceuncert{GW200115A}$ & $\masstwosourceuncert{GW200115A}$ & $\chieffinfinityonlyprecavguncert{GW200115A}$ & $\luminositydistanceuncert{GW200115A}$ & $\redshiftuncert{GW200115A}$ & $\finalmasssourceuncert{GW200115A}$ & $\finalspinuncert{GW200115A}$ & $\skyarea{GW200115A}$ & $\networkmatchedfiltersnrIMRPuncert{GW200115A}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW200128C} & $\totalmasssourceuncert{GW200128C}$ & $\chirpmasssourceuncert{GW200128C}$ & $\massonesourceuncert{GW200128C}$ & $\masstwosourceuncert{GW200128C}$ & $\chieffinfinityonlyprecavguncert{GW200128C}$ & $\luminositydistanceuncert{GW200128C}$ & $\redshiftuncert{GW200128C}$ & $\finalmasssourceuncert{GW200128C}$ & $\finalspinuncert{GW200128C}$ & $\skyarea{GW200128C}$ & $\networkmatchedfiltersnrIMRPuncert{GW200128C}$\\
\FULLNAME{GW200129D} & $\totalmasssourceuncert{GW200129D}$ & $\chirpmasssourceuncert{GW200129D}$ & $\massonesourceuncert{GW200129D}$ & $\masstwosourceuncert{GW200129D}$ & $\chieffinfinityonlyprecavguncert{GW200129D}$ & $\luminositydistanceuncert{GW200129D}$ & $\redshiftuncert{GW200129D}$ & $\finalmasssourceuncert{GW200129D}$ & $\finalspinuncert{GW200129D}$ & $\skyarea{GW200129D}$ & $\networkmatchedfiltersnrIMRPuncert{GW200129D}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW200202F} & $\totalmasssourceuncert{GW200202F}$ & $\chirpmasssourceuncert{GW200202F}$ & $\massonesourceuncert{GW200202F}$ & $\masstwosourceuncert{GW200202F}$ & $\chieffinfinityonlyprecavguncert{GW200202F}$ & $\luminositydistanceuncert{GW200202F}$ & $\redshiftuncert{GW200202F}$ & $\finalmasssourceuncert{GW200202F}$ & $\finalspinuncert{GW200202F}$ & $\skyarea{GW200202F}$ & $\networkmatchedfiltersnrIMRPuncert{GW200202F}$\\
\FULLNAME{GW200208G} & $\totalmasssourceuncert{GW200208G}$ & $\chirpmasssourceuncert{GW200208G}$ & $\massonesourceuncert{GW200208G}$ & $\masstwosourceuncert{GW200208G}$ & $\chieffinfinityonlyprecavguncert{GW200208G}$ & $\luminositydistanceuncert{GW200208G}$ & $\redshiftuncert{GW200208G}$ & $\finalmasssourceuncert{GW200208G}$ & $\finalspinuncert{GW200208G}$ & $\skyarea{GW200208G}$ & $\networkmatchedfiltersnrIMRPuncert{GW200208G}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW200208K} & $\totalmasssourceuncert{GW200208K}$ & $\chirpmasssourceuncert{GW200208K}$ & $\massonesourceuncert{GW200208K}$ & $\masstwosourceuncert{GW200208K}$ & $\chieffinfinityonlyprecavguncert{GW200208K}$ & $\luminositydistanceuncert{GW200208K}$ & $\redshiftuncert{GW200208K}$ & $\finalmasssourceuncert{GW200208K}$ & $\finalspinuncert{GW200208K}$ & $\skyarea{GW200208K}$ & $\networkmatchedfiltersnrIMRPuncert{GW200208K}$\\
\FULLNAME{GW200209E} & $\totalmasssourceuncert{GW200209E}$ & $\chirpmasssourceuncert{GW200209E}$ & $\massonesourceuncert{GW200209E}$ & $\masstwosourceuncert{GW200209E}$ & $\chieffinfinityonlyprecavguncert{GW200209E}$ & $\luminositydistanceuncert{GW200209E}$ & $\redshiftuncert{GW200209E}$ & $\finalmasssourceuncert{GW200209E}$ & $\finalspinuncert{GW200209E}$ & $\skyarea{GW200209E}$ & $\networkmatchedfiltersnrIMRPuncert{GW200209E}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW200210B} & $\totalmasssourceuncert{GW200210B}$ & $\chirpmasssourceuncert{GW200210B}$ & $\massonesourceuncert{GW200210B}$ & $\masstwosourceuncert{GW200210B}$ & $\chieffinfinityonlyprecavguncert{GW200210B}$ & $\luminositydistanceuncert{GW200210B}$ & $\redshiftuncert{GW200210B}$ & $\finalmasssourceuncert{GW200210B}$ & $\finalspinuncert{GW200210B}$ & $\skyarea{GW200210B}$ & $\networkmatchedfiltersnrIMRPuncert{GW200210B}$\\
\FULLNAME{GW200216G} & $\totalmasssourceuncert{GW200216G}$ & $\chirpmasssourceuncert{GW200216G}$ & $\massonesourceuncert{GW200216G}$ & $\masstwosourceuncert{GW200216G}$ & $\chieffinfinityonlyprecavguncert{GW200216G}$ & $\luminositydistanceuncert{GW200216G}$ & $\redshiftuncert{GW200216G}$ & $\finalmasssourceuncert{GW200216G}$ & $\finalspinuncert{GW200216G}$ & $\skyarea{GW200216G}$ & $\networkmatchedfiltersnrIMRPuncert{GW200216G}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW200219D} & $\totalmasssourceuncert{GW200219D}$ & $\chirpmasssourceuncert{GW200219D}$ & $\massonesourceuncert{GW200219D}$ & $\masstwosourceuncert{GW200219D}$ & $\chieffinfinityonlyprecavguncert{GW200219D}$ & $\luminositydistanceuncert{GW200219D}$ & $\redshiftuncert{GW200219D}$ & $\finalmasssourceuncert{GW200219D}$ & $\finalspinuncert{GW200219D}$ & $\skyarea{GW200219D}$ & $\networkmatchedfiltersnrIMRPuncert{GW200219D}$\\
\FULLNAME{GW200220E} & $\totalmasssourceuncert{GW200220E}$ & $\chirpmasssourceuncert{GW200220E}$ & $\massonesourceuncert{GW200220E}$ & $\masstwosourceuncert{GW200220E}$ & $\chieffinfinityonlyprecavguncert{GW200220E}$ & $\luminositydistanceuncert{GW200220E}$ & $\redshiftuncert{GW200220E}$ & $\finalmasssourceuncert{GW200220E}$ & $\finalspinuncert{GW200220E}$ & $\skyarea{GW200220E}$ & $\networkmatchedfiltersnrIMRPuncert{GW200220E}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW200220H} & $\totalmasssourceuncert{GW200220H}$ & $\chirpmasssourceuncert{GW200220H}$ & $\massonesourceuncert{GW200220H}$ & $\masstwosourceuncert{GW200220H}$ & $\chieffinfinityonlyprecavguncert{GW200220H}$ & $\luminositydistanceuncert{GW200220H}$ & $\redshiftuncert{GW200220H}$ & $\finalmasssourceuncert{GW200220H}$ & $\finalspinuncert{GW200220H}$ & $\skyarea{GW200220H}$ & $\networkmatchedfiltersnrIMRPuncert{GW200220H}$\\
\FULLNAME{GW200224H} & $\totalmasssourceuncert{GW200224H}$ & $\chirpmasssourceuncert{GW200224H}$ & $\massonesourceuncert{GW200224H}$ & $\masstwosourceuncert{GW200224H}$ & $\chieffinfinityonlyprecavguncert{GW200224H}$ & $\luminositydistanceuncert{GW200224H}$ & $\redshiftuncert{GW200224H}$ & $\finalmasssourceuncert{GW200224H}$ & $\finalspinuncert{GW200224H}$ & $\skyarea{GW200224H}$ & $\networkmatchedfiltersnrIMRPuncert{GW200224H}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW200225B} & $\totalmasssourceuncert{GW200225B}$ & $\chirpmasssourceuncert{GW200225B}$ & $\massonesourceuncert{GW200225B}$ & $\masstwosourceuncert{GW200225B}$ & $\chieffinfinityonlyprecavguncert{GW200225B}$ & $\luminositydistanceuncert{GW200225B}$ & $\redshiftuncert{GW200225B}$ & $\finalmasssourceuncert{GW200225B}$ & $\finalspinuncert{GW200225B}$ & $\skyarea{GW200225B}$ & $\networkmatchedfiltersnrIMRPuncert{GW200225B}$\\
\FULLNAME{GW200302A} & $\totalmasssourceuncert{GW200302A}$ & $\chirpmasssourceuncert{GW200302A}$ & $\massonesourceuncert{GW200302A}$ & $\masstwosourceuncert{GW200302A}$ & $\chieffinfinityonlyprecavguncert{GW200302A}$ & $\luminositydistanceuncert{GW200302A}$ & $\redshiftuncert{GW200302A}$ & $\finalmasssourceuncert{GW200302A}$ & $\finalspinuncert{GW200302A}$ & $\skyarea{GW200302A}$ & $\networkmatchedfiltersnrIMRPuncert{GW200302A}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW200306A} & $\totalmasssourceuncert{GW200306A}$ & $\chirpmasssourceuncert{GW200306A}$ & $\massonesourceuncert{GW200306A}$ & $\masstwosourceuncert{GW200306A}$ & $\chieffinfinityonlyprecavguncert{GW200306A}$ & $\luminositydistanceuncert{GW200306A}$ & $\redshiftuncert{GW200306A}$ & $\finalmasssourceuncert{GW200306A}$ & $\finalspinuncert{GW200306A}$ & $\skyarea{GW200306A}$ & $\networkmatchedfiltersnrIMRPuncert{GW200306A}$\\
\FULLNAME{GW200308G}$^{*}$ & $\totalmasssourceuncertwithcut{GW200308G}$ & $\chirpmasssourceuncertwithcut{GW200308G}$ & $\massonesourceuncertwithcut{GW200308G}$ & $\masstwosourceuncertwithcut{GW200308G}$ & $\chieffinfinityonlyprecavguncertwithcut{GW200308G}$ & $\luminositydistanceuncertwithcut{GW200308G}$ & $\redshiftuncertwithcut{GW200308G}$ & $\finalmasssourceuncertwithcut{GW200308G}$ & $\finalspinuncertwithcut{GW200308G}$ & $\skyareawithcut{GW200308G}$ & $\networkmatchedfiltersnrIMRPuncertwithcut{GW200308G}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW200311L} & $\totalmasssourceuncert{GW200311L}$ & $\chirpmasssourceuncert{GW200311L}$ & $\massonesourceuncert{GW200311L}$ & $\masstwosourceuncert{GW200311L}$ & $\chieffinfinityonlyprecavguncert{GW200311L}$ & $\luminositydistanceuncert{GW200311L}$ & $\redshiftuncert{GW200311L}$ & $\finalmasssourceuncert{GW200311L}$ & $\finalspinuncert{GW200311L}$ & $\skyarea{GW200311L}$ & $\networkmatchedfiltersnrIMRPuncert{GW200311L}$\\
\FULLNAME{GW200316I} & $\totalmasssourceuncert{GW200316I}$ & $\chirpmasssourceuncert{GW200316I}$ & $\massonesourceuncert{GW200316I}$ & $\masstwosourceuncert{GW200316I}$ & $\chieffinfinityonlyprecavguncert{GW200316I}$ & $\luminositydistanceuncert{GW200316I}$ & $\redshiftuncert{GW200316I}$ & $\finalmasssourceuncert{GW200316I}$ & $\finalspinuncert{GW200316I}$ & $\skyarea{GW200316I}$ & $\networkmatchedfiltersnrIMRPuncert{GW200316I}$\\
\makebox[0pt][l]{\fboxsep0pt\colorbox{lightgray}{\mystrut\hspace*{1.0\linewidth}}}\!\!
\FULLNAME{GW200322G}$^{*}$ & $\totalmasssourceuncertwithcut{GW200322G}$ & $\chirpmasssourceuncertwithcut{GW200322G}$ & $\massonesourceuncertwithcut{GW200322G}$ & $\masstwosourceuncertwithcut{GW200322G}$ & $\chieffinfinityonlyprecavguncertwithcut{GW200322G}$ & $\luminositydistanceuncertwithcut{GW200322G}$ & $\redshiftuncertwithcut{GW200322G}$ & $\finalmasssourceuncertwithcut{GW200322G}$ & $\finalspinuncertwithcut{GW200322G}$ & $\skyareawithcut{GW200322G}$ & $\networkmatchedfiltersnrIMRPuncertwithcut{GW200322G}$\\
\end{tabular}\end{ruledtabular}

==> inst_table_h1_l1.tex <==
\begin{ruledtabular}
\begin{tabularx}{\textwidth}{@{\extracolsep{\fill}}l l l l l}Parameter & O1 & O2 & O3a & O3b \\ \hline
Input laser power  & \HANFORDPOWERONE{} (H), \LIVINGSTONPOWERONE{} (L) & \HANFORDPOWERTWO{} (H), \LIVINGSTONPOWERTWO{} (L) & \HANFORDPOWERTHREEA{} (H), \LIVINGSTONPOWERTHREEA{} (L) & \HANFORDPOWER{} (H), \LIVINGSTONPOWER{} (L) \\ 
Power recycling gain   & \HANFORDPRGONE{} (H), \LIVINGSTONPRGONE{} (L) & \HANFORDPRGTWO{} (H), \LIVINGSTONPRGTWO{} (L) & \HANFORDPRGTHREEA{} (H), \LIVINGSTONPRGTHREEA{} (L) & \HANFORDPRG{} (H), \LIVINGSTONPRG{} (L) \\ 
Signal recycling       & \checkmark  &  \checkmark               & \checkmark                &  \checkmark \\ 
Squeezing              & $\times$  & $\times$                & \checkmark           & \checkmark  \\ 
Suspension type        & Monolithic & Monolithic & Monolithic & Monolithic \\ 
\end{tabularx}
\end{ruledtabular}


==> inst_table_v1.tex <==
\begin{ruledtabular}
\begin{tabularx}{\textwidth}{@{\extracolsep{\fill}}l l l l}Parameter & O2 & O3a & O3b \\ \hline
Input laser power  & \VIRGOPOWERTWO{} & \VIRGOPOWERTHREEA{} & \VIRGOPOWER{}   \\
Power recycling gain   & \VIRGOPRGTWO{} & \VIRGOPRGTHREEA{} & \VIRGOPRG{}   \\
Signal recycling       & $\times$  &  $\times$               & $\times$                 \\ 
Squeezing              & $\times$                  & \checkmark           & \checkmark  \\ 
Suspension type        & Wire & Monolithic & Monolithic \\ 
\end{tabularx}
\end{ruledtabular}


==> name_macros.tex <==
\DeclareRobustCommand{\SNAME}[1]{\IfEqCase{#1}{{GW200322A}{S200322ab}{GW200316A}{S200316bj}{GW200311B}{S200311bg}{GW200308A}{S200308bl}{GW200306A}{S200306ak}{GW200302A}{S200302c}{GW200225A}{S200225q}{GW200224A}{S200224ca}{GW200220A}{S200220ad}{GW200219A}{S200219ac}{GW200218A}{S200218al}{GW200216A}{S200216br}{GW200210A}{S200210ba}{GW200209A}{S200209ab}{GW200208B}{S200208am}{GW200208A}{S200208q}{GW200202A}{S200202ac}{GW200129A}{S200129m}{GW200128A}{S200128d}{GW200115A}{S200115j}{GW200112A}{S200112r}{GW200105A}{S200105ae}{GW191230A}{S191230an}{GW191222A}{S191222n}{GW191219A}{S191219ax}{GW191216A}{S191216ap}{GW191215A}{S191215w}{GW191213A}{S191213bb}{GW191204B}{S191204r}{GW191204A}{S191204h}{GW191129A}{S191129u}{GW191127A}{S191127p}{GW191126A}{S191126l}{GW191113A}{S191113q}{GW191109A}{S191109d}{GW191105A}{S191105e}{GW191103A}{S191103a}{200311A}{S200311ba}{200219B}{S200219bj}{200201A}{S200201bh}{200121A}{S200121aa}{191118A}{S191118ae}}}
\DeclareRobustCommand{\FULLNAME}[1]{\IfEqCase{#1}{{GW200322A}{GW200322\_091133}{GW200316A}{GW200316\_215756}{GW200311B}{GW200311\_115853}{GW200308A}{GW200308\_173609}{GW200306A}{GW200306\_093714}{GW200302A}{GW200302\_015811}{GW200225A}{GW200225\_060421}{GW200224A}{GW200224\_222234}{GW200220A}{GW200220\_061928}{GW200219A}{GW200219\_094415}{GW200218A}{GW200218\_100521}{GW200216A}{GW200216\_220804}{GW200210A}{GW200210\_092254}{GW200209A}{GW200209\_085452}{GW200208B}{GW200208\_222618}{GW200208A}{GW200208\_130117}{GW200202A}{GW200202\_154313}{GW200129A}{GW200129\_065458}{GW200128A}{GW200128\_022011}{GW200115A}{GW200115\_042309}{GW200112A}{GW200112\_155838}{GW200105A}{GW200105\_162426}{GW191230A}{GW191230\_180458}{GW191222A}{GW191222\_033537}{GW191219A}{GW191219\_163120}{GW191216A}{GW191216\_213338}{GW191215A}{GW191215\_223052}{GW191213A}{GW191213\_194013}{GW191204B}{GW191204\_171526}{GW191204A}{GW191204\_110529}{GW191129A}{GW191129\_134029}{GW191127A}{GW191127\_050227}{GW191126A}{GW191126\_115259}{GW191113A}{GW191113\_071753}{GW191109A}{GW191109\_010717}{GW191105A}{GW191105\_143521}{GW191103A}{GW191103\_012549}{200311A}{200311\_103121}{200219B}{200219\_201407}{200201A}{200201\_203549}{200121A}{200121\_031748}{191118A}{191118\_212859}}}
\DeclareRobustCommand{\NNAME}[1]{\IfEqCase{#1}{{GW200322A}{GW200322\_091133}{GW200316A}{GW200316\_215756}{GW200311B}{GW200311\_115853}{GW200308A}{GW200308\_173609}{GW200306A}{GW200306\_093714}{GW200302A}{GW200302\_015811}{GW200225A}{GW200225\_060421}{GW200224A}{GW200224\_222234}{GW200220A}{GW200220\_061928}{GW200219A}{GW200219\_094415}{GW200218A}{GW200218\_100521}{GW200216A}{GW200216\_220804}{GW200210A}{GW200210\_092254}{GW200209A}{GW200209\_085452}{GW200208B}{GW200208\_222618}{GW200208A}{GW200208\_130117}{GW200202A}{GW200202\_154313}{GW200129A}{GW200129\_065458}{GW200128A}{GW200128\_022011}{GW200115A}{GW200115}{GW200112A}{GW200112\_155838}{GW200105A}{GW200105}{GW191230A}{GW191230\_180458}{GW191222A}{GW191222\_033537}{GW191219A}{GW191219\_163120}{GW191216A}{GW191216\_213338}{GW191215A}{GW191215\_223052}{GW191213A}{GW191213\_194013}{GW191204B}{GW191204\_171526}{GW191204A}{GW191204\_110529}{GW191129A}{GW191129\_134029}{GW191127A}{GW191127\_050227}{GW191126A}{GW191126\_115259}{GW191113A}{GW191113\_071753}{GW191109A}{GW191109\_010717}{GW191105A}{GW191105\_143521}{GW191103A}{GW191103\_012549}{200311A}{200311\_103121}{200219B}{200219\_201407}{200201A}{200201\_203549}{200121A}{200121\_031748}{191118A}{191118\_212859}}}
\DeclareRobustCommand{\MINIMALNAME}[1]{\IfEqCase{#1}{{GW200322A}{GW200322}{GW200316A}{GW200316}{GW200311B}{GW200311\_11}{GW200308A}{GW200308}{GW200306A}{GW200306}{GW200302A}{GW200302}{GW200225A}{GW200225}{GW200224A}{GW200224}{GW200220A}{GW200220}{GW200219A}{GW200219\_09}{GW200218A}{GW200218}{GW200216A}{GW200216}{GW200210A}{GW200210}{GW200209A}{GW200209}{GW200208B}{GW200208\_22}{GW200208A}{GW200208\_13}{GW200202A}{GW200202}{GW200129A}{GW200129}{GW200128A}{GW200128}{GW200115A}{GW200115}{GW200112A}{GW200112}{GW200105A}{GW200105}{GW191230A}{GW191230}{GW191222A}{GW191222}{GW191219A}{GW191219}{GW191216A}{GW191216}{GW191215A}{GW191215}{GW191213A}{GW191213}{GW191204B}{GW191204\_17}{GW191204A}{GW191204\_11}{GW191129A}{GW191129}{GW191127A}{GW191127}{GW191126A}{GW191126}{GW191113A}{GW191113}{GW191109A}{GW191109}{GW191105A}{GW191105}{GW191103A}{GW191103}{200311A}{200311\_10}{200219B}{200219\_20}{200201A}{200201}{200121A}{200121}{191118A}{191118}}}


==> superlative_macros_with_cuts.tex <==

    \newcommand{\luminositydistanceleastwithcut}{200105F}

    \newcommand{\luminositydistanceleastpercentwithcut}{48}

    \newcommand{\luminositydistancemostwithcut}{GW200220E}

    \newcommand{\luminositydistancemostpercentwithcut}{33}

    \newcommand{\luminositydistanceleastsecondwithcut}{GW200115A}

    \newcommand{\luminositydistanceleastpercentsecondwithcut}{31}

    \newcommand{\luminositydistancemostsecondwithcut}{GW200322G}

    \newcommand{\luminositydistancemostpercentsecondwithcut}{25}

    
    \newcommand{\massonesourceleastwithcut}{GW200115A}

    \newcommand{\massonesourceleastpercentwithcut}{96}

    \newcommand{\massonesourcemostwithcut}{GW200220E}

    \newcommand{\massonesourcemostpercentwithcut}{63}

    \newcommand{\massonesourceleastsecondwithcut}{200105F}

    \newcommand{\massonesourceleastpercentsecondwithcut}{ 3}

    \newcommand{\massonesourcemostsecondwithcut}{GW200208K}

    \newcommand{\massonesourcemostpercentsecondwithcut}{17}

    
    \newcommand{\masstwosourceleastwithcut}{GW191219E}

    \newcommand{\masstwosourceleastpercentwithcut}{93}

    \newcommand{\masstwosourcemostwithcut}{GW200220E}

    \newcommand{\masstwosourcemostpercentwithcut}{77}

    \newcommand{\masstwosourceleastsecondwithcut}{GW200115A}

    \newcommand{\masstwosourceleastpercentsecondwithcut}{ 7}

    \newcommand{\masstwosourcemostsecondwithcut}{GW191109A}

    \newcommand{\masstwosourcemostpercentsecondwithcut}{19}

    
    \newcommand{\totalmasssourceleastwithcut}{GW200115A}

    \newcommand{\totalmasssourceleastpercentwithcut}{99}

    \newcommand{\totalmasssourcemostwithcut}{GW200220E}

    \newcommand{\totalmasssourcemostpercentwithcut}{87}

    \newcommand{\totalmasssourceleastsecondwithcut}{200105F}

    \newcommand{\totalmasssourceleastpercentsecondwithcut}{ 1}

    \newcommand{\totalmasssourcemostsecondwithcut}{GW191109A}

    \newcommand{\totalmasssourcemostpercentsecondwithcut}{ 5}

    
    \newcommand{\chirpmasssourceleastwithcut}{GW200115A}

    \newcommand{\chirpmasssourceleastpercentwithcut}{100}

    \newcommand{\chirpmasssourcemostwithcut}{GW200220E}

    \newcommand{\chirpmasssourcemostpercentwithcut}{90}

    \newcommand{\chirpmasssourceleastsecondwithcut}{GW191219E}

    \newcommand{\chirpmasssourceleastpercentsecondwithcut}{ 0}

    \newcommand{\chirpmasssourcemostsecondwithcut}{GW191109A}

    \newcommand{\chirpmasssourcemostpercentsecondwithcut}{ 9}

    
    \newcommand{\massratioleastwithcut}{GW191219E}

    \newcommand{\massratioleastpercentwithcut}{100}

    \newcommand{\massratiomostwithcut}{GW200129D}

    \newcommand{\massratiomostpercentwithcut}{ 6}

    \newcommand{\massratioleastsecondwithcut}{GW200210B}

    \newcommand{\massratioleastpercentsecondwithcut}{ 0}

    \newcommand{\massratiomostsecondwithcut}{GW200311L}

    \newcommand{\massratiomostpercentsecondwithcut}{ 6}

    
    \newcommand{\chieffleastwithcut}{GW191109A}

    \newcommand{\chieffleastpercentwithcut}{33}

    \newcommand{\chieffmostwithcut}{GW200308G}

    \newcommand{\chieffmostpercentwithcut}{59}

    \newcommand{\chieffleastsecondwithcut}{GW200115A}

    \newcommand{\chieffleastpercentsecondwithcut}{17}

    \newcommand{\chieffmostsecondwithcut}{GW200208K}

    \newcommand{\chieffmostpercentsecondwithcut}{27}

    
    \newcommand{\chieffinfinityonlyprecavgleastwithcut}{GW191109A}

    \newcommand{\chieffinfinityonlyprecavgleastpercentwithcut}{33}

    \newcommand{\chieffinfinityonlyprecavgmostwithcut}{GW200308G}

    \newcommand{\chieffinfinityonlyprecavgmostpercentwithcut}{59}

    \newcommand{\chieffinfinityonlyprecavgleastsecondwithcut}{GW200115A}

    \newcommand{\chieffinfinityonlyprecavgleastpercentsecondwithcut}{17}

    \newcommand{\chieffinfinityonlyprecavgmostsecondwithcut}{GW200208K}

    \newcommand{\chieffinfinityonlyprecavgmostpercentsecondwithcut}{27}

    
    \newcommand{\chipleastwithcut}{GW191219E}

    \newcommand{\chipleastpercentwithcut}{23}

    \newcommand{\chipmostwithcut}{GW200129D}

    \newcommand{\chipmostpercentwithcut}{11}

    \newcommand{\chipleastsecondwithcut}{200105F}

    \newcommand{\chipleastpercentsecondwithcut}{23}

    \newcommand{\chipmostsecondwithcut}{GW191127B}

    \newcommand{\chipmostpercentsecondwithcut}{ 8}

    
    \newcommand{\chipinfinityonlyprecavgleastwithcut}{200105F}

    \newcommand{\chipinfinityonlyprecavgleastpercentwithcut}{23}

    \newcommand{\chipinfinityonlyprecavgmostwithcut}{GW200129D}

    \newcommand{\chipinfinityonlyprecavgmostpercentwithcut}{11}

    \newcommand{\chipinfinityonlyprecavgleastsecondwithcut}{GW191219E}

    \newcommand{\chipinfinityonlyprecavgleastpercentsecondwithcut}{23}

    \newcommand{\chipinfinityonlyprecavgmostsecondwithcut}{GW191127B}

    \newcommand{\chipinfinityonlyprecavgmostpercentsecondwithcut}{ 8}

    
    \newcommand{\finalspinleastwithcut}{GW191219E}

    \newcommand{\finalspinleastpercentwithcut}{99}

    \newcommand{\finalspinmostwithcut}{GW200308G}

    \newcommand{\finalspinmostpercentwithcut}{54}

    \newcommand{\finalspinleastsecondwithcut}{GW200210B}

    \newcommand{\finalspinleastpercentsecondwithcut}{ 0}

    \newcommand{\finalspinmostsecondwithcut}{GW200208K}

    \newcommand{\finalspinmostpercentsecondwithcut}{29}

    
    \newcommand{\luminositydistanceleastBBHwithcut}{GW191216G}

    \newcommand{\luminositydistanceleastpercentBBHwithcut}{69}

    \newcommand{\luminositydistancemostBBHwithcut}{GW200220E}

    \newcommand{\luminositydistancemostpercentBBHwithcut}{33}

    \newcommand{\luminositydistanceleastsecondBBHwithcut}{GW200202F}

    \newcommand{\luminositydistanceleastpercentsecondBBHwithcut}{26}

    \newcommand{\luminositydistancemostsecondBBHwithcut}{GW200322G}

    \newcommand{\luminositydistancemostpercentsecondBBHwithcut}{25}

    
    \newcommand{\massonesourceleastBBHwithcut}{GW200202F}

    \newcommand{\massonesourceleastpercentBBHwithcut}{35}

    \newcommand{\massonesourcemostBBHwithcut}{GW200220E}

    \newcommand{\massonesourcemostpercentBBHwithcut}{63}

    \newcommand{\massonesourceleastsecondBBHwithcut}{GW191129G}

    \newcommand{\massonesourceleastpercentsecondBBHwithcut}{27}

    \newcommand{\massonesourcemostsecondBBHwithcut}{GW200208K}

    \newcommand{\massonesourcemostpercentsecondBBHwithcut}{17}

    
    \newcommand{\masstwosourceleastBBHwithcut}{GW191113B}

    \newcommand{\masstwosourceleastpercentBBHwithcut}{40}

    \newcommand{\masstwosourcemostBBHwithcut}{GW200220E}

    \newcommand{\masstwosourcemostpercentBBHwithcut}{76}

    \newcommand{\masstwosourceleastsecondBBHwithcut}{GW191129G}

    \newcommand{\masstwosourceleastpercentsecondBBHwithcut}{16}

    \newcommand{\masstwosourcemostsecondBBHwithcut}{GW191109A}

    \newcommand{\masstwosourcemostpercentsecondBBHwithcut}{19}

    
    \newcommand{\totalmasssourceleastBBHwithcut}{GW191129G}

    \newcommand{\totalmasssourceleastpercentBBHwithcut}{49}

    \newcommand{\totalmasssourcemostBBHwithcut}{GW200220E}

    \newcommand{\totalmasssourcemostpercentBBHwithcut}{87}

    \newcommand{\totalmasssourceleastsecondBBHwithcut}{GW200202F}

    \newcommand{\totalmasssourceleastpercentsecondBBHwithcut}{40}

    \newcommand{\totalmasssourcemostsecondBBHwithcut}{GW191109A}

    \newcommand{\totalmasssourcemostpercentsecondBBHwithcut}{ 5}

    
    \newcommand{\chirpmasssourceleastBBHwithcut}{GW191129G}

    \newcommand{\chirpmasssourceleastpercentBBHwithcut}{70}

    \newcommand{\chirpmasssourcemostBBHwithcut}{GW200220E}

    \newcommand{\chirpmasssourcemostpercentBBHwithcut}{90}

    \newcommand{\chirpmasssourceleastsecondBBHwithcut}{GW200202F}

    \newcommand{\chirpmasssourceleastpercentsecondBBHwithcut}{24}

    \newcommand{\chirpmasssourcemostsecondBBHwithcut}{GW191109A}

    \newcommand{\chirpmasssourcemostpercentsecondBBHwithcut}{ 9}

    
    \newcommand{\massratioleastBBHwithcut}{GW200208K}

    \newcommand{\massratioleastpercentBBHwithcut}{35}

    \newcommand{\massratiomostBBHwithcut}{GW200129D}

    \newcommand{\massratiomostpercentBBHwithcut}{ 6}

    \newcommand{\massratioleastsecondBBHwithcut}{GW191113B}

    \newcommand{\massratioleastpercentsecondBBHwithcut}{27}

    \newcommand{\massratiomostsecondBBHwithcut}{GW200311L}

    \newcommand{\massratiomostpercentsecondBBHwithcut}{ 6}

    
    \newcommand{\chieffleastBBHwithcut}{GW191109A}

    \newcommand{\chieffleastpercentBBHwithcut}{39}

    \newcommand{\chieffmostBBHwithcut}{GW200308G}

    \newcommand{\chieffmostpercentBBHwithcut}{59}

    \newcommand{\chieffleastsecondBBHwithcut}{GW200209E}

    \newcommand{\chieffleastpercentsecondBBHwithcut}{ 9}

    \newcommand{\chieffmostsecondBBHwithcut}{GW200208K}

    \newcommand{\chieffmostpercentsecondBBHwithcut}{27}

    
    \newcommand{\chieffinfinityonlyprecavgleastBBHwithcut}{GW191109A}

    \newcommand{\chieffinfinityonlyprecavgleastpercentBBHwithcut}{39}

    \newcommand{\chieffinfinityonlyprecavgmostBBHwithcut}{GW200308G}

    \newcommand{\chieffinfinityonlyprecavgmostpercentBBHwithcut}{59}

    \newcommand{\chieffinfinityonlyprecavgleastsecondBBHwithcut}{GW200209E}

    \newcommand{\chieffinfinityonlyprecavgleastpercentsecondBBHwithcut}{ 9}

    \newcommand{\chieffinfinityonlyprecavgmostsecondBBHwithcut}{GW200208K}

    \newcommand{\chieffinfinityonlyprecavgmostpercentsecondBBHwithcut}{27}

    
    \newcommand{\chipleastBBHwithcut}{GW191113B}

    \newcommand{\chipleastpercentBBHwithcut}{15}

    \newcommand{\chipmostBBHwithcut}{GW200129D}

    \newcommand{\chipmostpercentBBHwithcut}{11}

    \newcommand{\chipleastsecondBBHwithcut}{GW191105C}

    \newcommand{\chipleastpercentsecondBBHwithcut}{ 8}

    \newcommand{\chipmostsecondBBHwithcut}{GW191127B}

    \newcommand{\chipmostpercentsecondBBHwithcut}{ 8}

    
    \newcommand{\chipinfinityonlyprecavgleastBBHwithcut}{GW191113B}

    \newcommand{\chipinfinityonlyprecavgleastpercentBBHwithcut}{15}

    \newcommand{\chipinfinityonlyprecavgmostBBHwithcut}{GW200129D}

    \newcommand{\chipinfinityonlyprecavgmostpercentBBHwithcut}{11}

    \newcommand{\chipinfinityonlyprecavgleastsecondBBHwithcut}{GW191105C}

    \newcommand{\chipinfinityonlyprecavgleastpercentsecondBBHwithcut}{ 8}

    \newcommand{\chipinfinityonlyprecavgmostsecondBBHwithcut}{GW191127B}

    \newcommand{\chipinfinityonlyprecavgmostpercentsecondBBHwithcut}{ 8}

    
    \newcommand{\finalspinleastBBHwithcut}{GW191113B}

    \newcommand{\finalspinleastpercentBBHwithcut}{51}

    \newcommand{\finalspinmostBBHwithcut}{GW200308G}

    \newcommand{\finalspinmostpercentBBHwithcut}{54}

    \newcommand{\finalspinleastsecondBBHwithcut}{GW191109A}

    \newcommand{\finalspinleastpercentsecondBBHwithcut}{11}

    \newcommand{\finalspinmostsecondBBHwithcut}{GW200208K}

    \newcommand{\finalspinmostpercentsecondBBHwithcut}{29}

    
